Receiver Concepts and Resource Allocation for OSC Downlink Transmission

Voice services over Adaptive Multi-user channels on One Slot (VAMOS) has been standardized as an extension to the Global System for Mobile Communications (GSM). The aim of VAMOS is to increase the capacity of GSM, while maintaining backward compatibility with the legacy system. To this end, the Orthogonal Sub-channels (OSC) concept is employed, where two Gaussian minimum-shift keying (GMSK) signals are transmitted in the same time slot and with the same carrier frequency. To fully exploit the possible capacity gain of OSC, new receiver concepts are necessary. In contrast to the base station, where multiple antennas can be employed, the mobile station is typically equipped with only one receive antenna. Therefore, the downlink receiver design is a very challenging task. Different concepts for channel estimation, user separation, and equalization at the receiver of an OSC downlink transmission are introduced in this paper. Furthermore, the system capacity must be improved by suitable downlink power and resource allocation algorithms. Making realistic assumptions on the information available at the base station, an algorithm for joint power and radio resource allocation is proposed. Simulation results show the excellent performance of the proposed channel estimation algorithms, equalization schemes, and joint radio resource and power allocation algorithms in realistic VAMOS environments.

==> CRB_pimrc_1_h.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{015}[cl][cl]{\matlabtextA CRB GSM\hspace{-0.5em}}%
\psfrag{016}[cl][cl]{\matlabtextA Simulation\hspace{-0.5em}}%
\psfrag{017}[cl][cl]{\matlabtextA CRB\hspace{-0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextB $\mathrm{MSE}_{\vv{h}} \ \longrightarrow$}%
\psfrag{019}[tc][tc]{\matlabtextB $10 \log_{10} (\mathrm{SNR}) \ [\mathrm{dB}] \ \longrightarrow$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 15$}%
\psfrag{002}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{003}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{004}[ct][ct]{\matlabtextC $0$}%
\psfrag{005}[ct][ct]{\matlabtextC $5$}%
\psfrag{006}[ct][ct]{\matlabtextC $10$}%
\psfrag{007}[ct][ct]{\matlabtextC $15$}%
\psfrag{008}[ct][ct]{\matlabtextC $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextC $10^{-3}$}%
\psfrag{010}[rc][rc]{\matlabtextC $10^{-2}$}%
\psfrag{011}[rc][rc]{\matlabtextC $10^{-1}$}%
\psfrag{012}[rc][rc]{\matlabtextC $10^{0}$}%
\psfrag{013}[rc][rc]{\matlabtextC $10^{1}$}%
\psfrag{014}[rc][rc]{\matlabtextC $10^{2}$}%
%
%% </ytick>

==> MTS1_AFS59.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA $\mathrm{SCPIR} = -8~$dB\hspace{-0.5em}}%
\psfrag{013}[cl][cl]{\matlabtextA $\mathrm{SCPIR} = -4~$dB\hspace{-0.5em}}%
\psfrag{014}[cl][cl]{\matlabtextA $\mathrm{SCPIR} = 0~$dB\hspace{-0.5em}}%
\psfrag{015}[cl][cl]{\matlabtextA V-MIC\hspace{-0.5em}}%
\psfrag{016}[cl][cl]{\matlabtextA SIC\hspace{-0.5em}}%
\psfrag{017}[cl][cl]{\matlabtextA MIC\hspace{-0.5em}}%
\psfrag{018}[cl][cl]{\matlabtextA Joint MLSE\hspace{-0.5em}}%
\psfrag{019}[cl][cl]{\matlabtextA CEQ w/o OSC\hspace{-0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextB DL MTS-1, TCH/AFS 5.9, TU3iFH}%
\psfrag{021}[bc][bc]{\matlabtextB $\mathrm{FER}$ of user $o \ \longrightarrow$}%
\psfrag{022}[tc][tc]{\matlabtextB $10 \log_{10} ( \mathrm{SINR} )$~[dB]$\ \longrightarrow$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $5$}%
\psfrag{004}[ct][ct]{\matlabtextC $10$}%
\psfrag{005}[ct][ct]{\matlabtextC $15$}%
\psfrag{006}[ct][ct]{\matlabtextC $20$}%
\psfrag{007}[ct][ct]{\matlabtextC $25$}%
\psfrag{008}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextC $10^{-2}$}%
\psfrag{010}[rc][rc]{\matlabtextC $10^{-1}$}%
\psfrag{011}[rc][rc]{\matlabtextC $10^{0}$}%
%
%% </ytick>

==> MTS2_AFS59.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA $\mathrm{SCPIR} = -8~$dB\hspace{-0.5em}}%
\psfrag{011}[cl][cl]{\matlabtextA $\mathrm{SCPIR} = -4~$dB\hspace{-0.5em}}%
\psfrag{012}[cl][cl]{\matlabtextA $\mathrm{SCPIR} = 0~$dB\hspace{-0.5em}}%
\psfrag{013}[cl][cl]{\matlabtextA V-MIC\hspace{-0.5em}}%
\psfrag{014}[cl][cl]{\matlabtextA SIC\hspace{-0.5em}}%
\psfrag{015}[cl][cl]{\matlabtextA MIC\hspace{-0.5em}}%
\psfrag{016}[cl][cl]{\matlabtextA Joint MLSE\hspace{-0.5em}}%
\psfrag{017}[cl][cl]{\matlabtextA CEQ w/o OSC\hspace{-0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextB DL MTS-2, TCH/AFS 5.9, TU3iFH}%
\psfrag{019}[bc][bc]{\matlabtextB $\mathrm{FER}$ of user $o \ \longrightarrow$}%
\psfrag{020}[tc][tc]{\matlabtextB $10 \log_{10} ( \mathrm{SINR} )$~[dB]$\ \longrightarrow$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $5$}%
\psfrag{004}[ct][ct]{\matlabtextC $10$}%
\psfrag{005}[ct][ct]{\matlabtextC $15$}%
\psfrag{006}[ct][ct]{\matlabtextC $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $10^{-2}$}%
\psfrag{008}[rc][rc]{\matlabtextC $10^{-1}$}%
\psfrag{009}[rc][rc]{\matlabtextC $10^{0}$}%
%
%% </ytick>

==> SAIC_vs_SIC_vs_VMIC_no_DTX_10_dB_AHS_FER.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA no-VAMOS\hspace{0.5em}}%
\psfrag{015}[cl][cl]{\matlabtextA VAMOS V-MIC\hspace{0.5em}}%
\psfrag{016}[cl][cl]{\matlabtextA VAMOS SIC\hspace{0.5em}}%
\psfrag{017}[cl][cl]{\matlabtextA VAMOS MIC\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextB AHS 5.9}%
\psfrag{019}[bc][bc]{\matlabtextB $\mathrm{FER}$ $\longrightarrow$}%
\psfrag{020}[tc][tc]{\matlabtextB $N_\mathrm{user} \ \longrightarrow$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $5$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $15$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
\psfrag{004}[ct][ct]{\matlabtextC $25$}%
\psfrag{005}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $0$}%
\psfrag{007}[rc][rc]{\matlabtextC $0.01$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.02$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.03$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.04$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.05$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.06$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.07$}%
%
%% </ytick>

==> SAIC_vs_SIC_vs_VMIC_no_DTX_10_dB_AHS_power.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{015}[cl][cl]{\matlabtextA no-VAMOS\hspace{0.5em}}%
\psfrag{016}[cl][cl]{\matlabtextA VAMOS V-MIC\hspace{0.5em}}%
\psfrag{017}[cl][cl]{\matlabtextA VAMOS SIC\hspace{0.5em}}%
\psfrag{018}[cl][cl]{\matlabtextA VAMOS MIC\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextB AHS 5.9}%
\psfrag{020}[bc][bc]{\matlabtextB $\mathrm{power~[dBm]}$ $\longrightarrow$}%
\psfrag{021}[tc][tc]{\matlabtextB $N_\mathrm{user} \ \longrightarrow$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $5$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $15$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
\psfrag{004}[ct][ct]{\matlabtextC $25$}%
\psfrag{005}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $18$}%
\psfrag{007}[rc][rc]{\matlabtextC $18.5$}%
\psfrag{008}[rc][rc]{\matlabtextC $19$}%
\psfrag{009}[rc][rc]{\matlabtextC $19.5$}%
\psfrag{010}[rc][rc]{\matlabtextC $20$}%
\psfrag{011}[rc][rc]{\matlabtextC $20.5$}%
\psfrag{012}[rc][rc]{\matlabtextC $21$}%
\psfrag{013}[rc][rc]{\matlabtextC $21.5$}%
\psfrag{014}[rc][rc]{\matlabtextC $22$}%
%
%% </ytick>

==> SAIC_vs_SIC_vs_VMIC_with_DTX_10_dB_AHS_FER.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA no-VAMOS\hspace{0.5em}}%
\psfrag{015}[cl][cl]{\matlabtextA VAMOS V-MIC\hspace{0.5em}}%
\psfrag{016}[cl][cl]{\matlabtextA VAMOS SIC\hspace{0.5em}}%
\psfrag{017}[cl][cl]{\matlabtextA VAMOS MIC\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextB AHS 5.9, DTX 40 \%}%
\psfrag{019}[bc][bc]{\matlabtextB $\mathrm{FER}$ $\longrightarrow$}%
\psfrag{020}[tc][tc]{\matlabtextB $N_\mathrm{user} \ \longrightarrow$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $5$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $15$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
\psfrag{004}[ct][ct]{\matlabtextC $25$}%
\psfrag{005}[ct][ct]{\matlabtextC $30$}%
\psfrag{006}[ct][ct]{\matlabtextC $35$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.005$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.01$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.015$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.02$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.025$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.03$}%
%
%% </ytick>

==> SAIC_vs_SIC_vs_VMIC_with_DTX_10_dB_AHS_power.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{017}[cl][cl]{\matlabtextA no-VAMOS\hspace{0.5em}}%
\psfrag{018}[cl][cl]{\matlabtextA VAMOS V-MIC\hspace{0.5em}}%
\psfrag{019}[cl][cl]{\matlabtextA VAMOS SIC\hspace{0.5em}}%
\psfrag{020}[cl][cl]{\matlabtextA VAMOS MIC\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB AHS 5.9, DTX 40 \%}%
\psfrag{022}[bc][bc]{\matlabtextB $\mathrm{power~[dBm]}$ $\longrightarrow$}%
\psfrag{023}[tc][tc]{\matlabtextB $N_\mathrm{user} \ \longrightarrow$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $5$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $15$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
\psfrag{004}[ct][ct]{\matlabtextC $25$}%
\psfrag{005}[ct][ct]{\matlabtextC $30$}%
\psfrag{006}[ct][ct]{\matlabtextC $35$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $18$}%
\psfrag{008}[rc][rc]{\matlabtextC $18.5$}%
\psfrag{009}[rc][rc]{\matlabtextC $19$}%
\psfrag{010}[rc][rc]{\matlabtextC $19.5$}%
\psfrag{011}[rc][rc]{\matlabtextC $20$}%
\psfrag{012}[rc][rc]{\matlabtextC $20.5$}%
\psfrag{013}[rc][rc]{\matlabtextC $21$}%
\psfrag{014}[rc][rc]{\matlabtextC $21.5$}%
\psfrag{015}[rc][rc]{\matlabtextC $22$}%
\psfrag{016}[rc][rc]{\matlabtextC $22.5$}%
%
%% </ytick>

==> hot_spot_AHS_FER.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{015}[cl][cl]{\matlabtextA no-VAMOS\hspace{0.5em}}%
\psfrag{016}[cl][cl]{\matlabtextA hot spot\hspace{0.5em}}%
\psfrag{017}[cl][cl]{\matlabtextA POOB\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextB AHS 5.9}%
\psfrag{019}[bc][bc]{\matlabtextB $\mathrm{FER}$ $\longrightarrow$}%
\psfrag{020}[tc][tc]{\matlabtextB $N_\mathrm{user} \ \longrightarrow$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $5$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $15$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
\psfrag{004}[ct][ct]{\matlabtextC $25$}%
\psfrag{005}[ct][ct]{\matlabtextC $30$}%
\psfrag{006}[ct][ct]{\matlabtextC $35$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.01$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.02$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.03$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.04$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.05$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.06$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.07$}%
%
%% </ytick>

==> hot_spot_AHS_power.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA no-VAMOS\hspace{0.5em}}%
\psfrag{017}[cl][cl]{\matlabtextA hot spot\hspace{0.5em}}%
\psfrag{018}[cl][cl]{\matlabtextA POOB\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextB AHS 5.9}%
\psfrag{020}[bc][bc]{\matlabtextB $\mathrm{power~[dBm]}$ $\longrightarrow$}%
\psfrag{021}[tc][tc]{\matlabtextB $N_\mathrm{user} \ \longrightarrow$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $5$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $15$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
\psfrag{004}[ct][ct]{\matlabtextC $25$}%
\psfrag{005}[ct][ct]{\matlabtextC $30$}%
\psfrag{006}[ct][ct]{\matlabtextC $35$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $18.5$}%
\psfrag{008}[rc][rc]{\matlabtextC $19$}%
\psfrag{009}[rc][rc]{\matlabtextC $19.5$}%
\psfrag{010}[rc][rc]{\matlabtextC $20$}%
\psfrag{011}[rc][rc]{\matlabtextC $20.5$}%
\psfrag{012}[rc][rc]{\matlabtextC $21$}%
\psfrag{013}[rc][rc]{\matlabtextC $21.5$}%
\psfrag{014}[rc][rc]{\matlabtextC $22$}%
\psfrag{015}[rc][rc]{\matlabtextC $22.5$}%
%
%% </ytick>

==> vamos_no_vamos_sim_pl_10_15_dB_transactions_AHS_FER.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA $\textrm{no-VAMOS } P_\mathrm{int} = 10$~dB\hspace{-0.7em}}%
\psfrag{015}[cl][cl]{\matlabtextA $\textrm{POOB } P_\mathrm{int} = 15$~dB\hspace{-0.7em}}%
\psfrag{016}[cl][cl]{\matlabtextA $\textrm{POOB } P_\mathrm{int} = 13$~dB\hspace{-0.7em}}%
\psfrag{017}[cl][cl]{\matlabtextA $\textrm{POOB } P_\mathrm{int} = 10$~dB\hspace{-0.7em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextB AHS 5.9}%
\psfrag{019}[bc][bc]{\matlabtextB $\mathrm{FER}$ $\longrightarrow$}%
\psfrag{020}[tc][tc]{\matlabtextB $N_\mathrm{user} \ \longrightarrow$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $5$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $15$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
\psfrag{004}[ct][ct]{\matlabtextC $25$}%
\psfrag{005}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $0$}%
\psfrag{007}[rc][rc]{\matlabtextC $0.01$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.02$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.03$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.04$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.05$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.06$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.07$}%
%
%% </ytick>

==> vamos_no_vamos_sim_pl_10_15_dB_transactions_AHS_power.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{015}[cl][cl]{\matlabtextA $\textrm{no-VAMOS } P_\mathrm{int} = 10$~dB\hspace{-0.7em}}%
\psfrag{016}[cl][cl]{\matlabtextA $\textrm{POOB } P_\mathrm{int} = 15$~dB\hspace{-0.7em}}%
\psfrag{017}[cl][cl]{\matlabtextA $\textrm{POOB } P_\mathrm{int} = 13$~dB\hspace{-0.7em}}%
\psfrag{018}[cl][cl]{\matlabtextA $\textrm{POOB } P_\mathrm{int} = 10$~dB\hspace{-0.7em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextB AHS 5.9}%
\psfrag{020}[bc][bc]{\matlabtextB $\mathrm{power~[dBm]}$ $\longrightarrow$}%
\psfrag{021}[tc][tc]{\matlabtextB $N_\mathrm{user} \ \longrightarrow$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $5$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $15$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
\psfrag{004}[ct][ct]{\matlabtextC $25$}%
\psfrag{005}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $18$}%
\psfrag{007}[rc][rc]{\matlabtextC $19$}%
\psfrag{008}[rc][rc]{\matlabtextC $20$}%
\psfrag{009}[rc][rc]{\matlabtextC $21$}%
\psfrag{010}[rc][rc]{\matlabtextC $22$}%
\psfrag{011}[rc][rc]{\matlabtextC $23$}%
\psfrag{012}[rc][rc]{\matlabtextC $24$}%
\psfrag{013}[rc][rc]{\matlabtextC $25$}%
\psfrag{014}[rc][rc]{\matlabtextC $26$}%
%
%% </ytick>

==> vamos_no_vamos_sim_pl_10_dB_transactions_AHS_FER.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{015}[cl][cl]{\matlabtextA $\textrm{no-VAMOS}$\hspace{-0.7em}}%
\psfrag{016}[cl][cl]{\matlabtextA $\textrm{POOB}$\hspace{-0.7em}}%
\psfrag{017}[cl][cl]{\matlabtextA $\textrm{user pairing}$\hspace{-0.7em}}%
\psfrag{018}[cl][cl]{\matlabtextA $\textrm{random pairing, SCPIR optim.}$\hspace{-0.7em}}%
\psfrag{019}[cl][cl]{\matlabtextA $\textrm{random pairing, SCPIR} = 0$~dB\hspace{-0.7em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextB AHS 5.9}%
\psfrag{021}[bc][bc]{\matlabtextB $\mathrm{FER}$ $\longrightarrow$}%
\psfrag{022}[tc][tc]{\matlabtextB $N_\mathrm{user} \ \longrightarrow$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $5$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $15$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
\psfrag{004}[ct][ct]{\matlabtextC $25$}%
\psfrag{005}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $0$}%
\psfrag{007}[rc][rc]{\matlabtextC $0.01$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.02$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.03$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.04$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.05$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.06$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.07$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.08$}%
%
%% </ytick>

==> vamos_no_vamos_sim_pl_10_dB_transactions_AHS_blocked_calls.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{018}[cl][cl]{\matlabtextA $\textrm{no-VAMOS}$\hspace{-0.7em}}%
\psfrag{019}[cl][cl]{\matlabtextA $\textrm{POOB}$\hspace{-0.7em}}%
\psfrag{020}[cl][cl]{\matlabtextA $\textrm{user pairing}$\hspace{-0.7em}}%
\psfrag{021}[cl][cl]{\matlabtextA $\textrm{random pairing, SCPIR optim.}$\hspace{-0.7em}}%
\psfrag{022}[cl][cl]{\matlabtextA $\textrm{random pairing, SCPIR} = 0$~dB\hspace{-0.7em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{023}[bc][bc]{\matlabtextB AHS 5.9}%
\psfrag{024}[bc][bc]{\matlabtextB $\mathrm{Ratio~of~blocked~calls}$ $\longrightarrow$}%
\psfrag{025}[tc][tc]{\matlabtextB $N_\mathrm{user} \ \longrightarrow$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $5$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $15$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
\psfrag{004}[ct][ct]{\matlabtextC $25$}%
\psfrag{005}[ct][ct]{\matlabtextC $30$}%
\psfrag{006}[ct][ct]{\matlabtextC $35$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{017}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> vamos_no_vamos_sim_pl_10_dB_transactions_AHS_power.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{017}[cl][cl]{\matlabtextA $\textrm{no-VAMOS}$\hspace{-0.7em}}%
\psfrag{018}[cl][cl]{\matlabtextA $\textrm{POOB}$\hspace{-0.7em}}%
\psfrag{019}[cl][cl]{\matlabtextA $\textrm{user pairing}$\hspace{-0.7em}}%
\psfrag{020}[cl][cl]{\matlabtextA $\textrm{random pairing, SCPIR optim.}$\hspace{-0.7em}}%
\psfrag{021}[cl][cl]{\matlabtextA $\textrm{random pairing, SCPIR} = 0$~dB\hspace{-0.7em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{022}[bc][bc]{\matlabtextB AHS 5.9}%
\psfrag{023}[bc][bc]{\matlabtextB $\mathrm{power~[dBm]}$ $\longrightarrow$}%
\psfrag{024}[tc][tc]{\matlabtextB $N_\mathrm{user} \ \longrightarrow$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $5$}%
\psfrag{001}[ct][ct]{\matlabtextC $10$}%
\psfrag{002}[ct][ct]{\matlabtextC $15$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
\psfrag{004}[ct][ct]{\matlabtextC $25$}%
\psfrag{005}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $18$}%
\psfrag{007}[rc][rc]{\matlabtextC $19$}%
\psfrag{008}[rc][rc]{\matlabtextC $20$}%
\psfrag{009}[rc][rc]{\matlabtextC $21$}%
\psfrag{010}[rc][rc]{\matlabtextC $22$}%
\psfrag{011}[rc][rc]{\matlabtextC $23$}%
\psfrag{012}[rc][rc]{\matlabtextC $24$}%
\psfrag{013}[rc][rc]{\matlabtextC $25$}%
\psfrag{014}[rc][rc]{\matlabtextC $26$}%
\psfrag{015}[rc][rc]{\matlabtextC $27$}%
\psfrag{016}[rc][rc]{\matlabtextC $28$}%
%
%% </ytick>
